The Distortion of Binomial Voting Defies Expectation

In computational social choice, the distortion of a voting rule quantifies the degree to which the rule overcomes limited preference information to select a socially desirable outcome. This concept has been investigated extensively, but only through a worst-case lens. Instead, we study the expected distortion of voting rules with respect to an underlying distribution over voter utilities. Our main contribution is the design and analysis of a novel and intuitive rule, binomial voting, which provides strong distribution-independent guarantees for both expected distortion and expected welfare.

==> preamble.tex <==
\usepackage[margin=1in]{geometry}
\usepackage{setspace}
\onehalfspacing
\usepackage{natbib}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\hypersetup{
    colorlinks = true,
    linkcolor = teal,
    citecolor = teal,
	urlcolor = teal
}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage[capitalize]{cleveref}
\def\proofname{proof}
\newtheorem{thm}{Theorem}[section]
\newtheorem{obs}[thm]{Observation}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{definition}[thm]{Definition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{property}[thm]{Property}
\newtheorem{remark}[thm]{Remark}
\newtheorem{claim}[thm]{Claim}
\newtheorem{note}[thm]{Note}
\newenvironment{proof}{\noindent\bf{Proof.}\rm}{\hfill$\blacksquare$\bigskip}
\newcommand{\qedsymbol}{\hfill\blacksquare}
\newcommand{\mc}{\mathcal}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\sw}{sw}
\DeclareMathOperator{\SW}{dsw}
\DeclareMathOperator{\wcdist}{distortion}
\DeclareMathOperator{\dist}{ddist}
\DeclareMathOperator{\invdist}{invddist}
\newcommand{\emdash}{\,---\,}
\DeclareMathOperator{\edmr}{edmr}
\DeclareMathOperator{\ewmr}{ewmr}
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\Var}{Var}
\DeclareMathOperator*{\bu}{\mathbf{u}}
\DeclareMathOperator*{\bsigma}{\boldsymbol{\sigma}}
\DeclareMathOperator*{\scr}{Score}
\DeclareMathOperator*{\brda}{Borda}
\DeclareMathOperator*{\bern}{Bern}
\DeclareMathOperator*{\bin}{Bin}
\DeclareMathOperator*{\unif}{Unif}
\DeclareMathOperator{\tha}{Top-Half}
\DeclareMathOperator{\bsr}{Binom}
\DeclareMathOperator{\gbsr}{GBinom}
\DeclareMathOperator{\plur}{Plurality}
\DeclareMathOperator{\samp}{Sampling}
\newcommand{\Dnm}{\mc{D}^{n \times m}}
\renewcommand{\epsilon}{\varepsilon}

==> proofs/EWMR_EDMR.tex <==
\section{Proof of Theorem~\ref{thm:neg}}\label{app:proof_of_neg}

\begin{lemma} \label{lem:atothebbounds}
    For $a \ge 0$ and integer $b \ge 2$ such that $ab \le 1/5$,
    \[
        1 - ab  \le (1-a)^b \le 1 - ab + (ab)^2
    \]
\end{lemma}

\begin{proof}
Expanding the binomial gives:
\[
    (1-a)^b =  1 - ab + \sum_{k=2}^b \binom{b}{k}(-a)^k 
\]
Examining the last terms, we have that
    \begin{align*}
       \left| \sum_{k=2}^b \binom{b}{k}(-a)^k\right| &\le  \frac{a^2b(b-1)}{2} + \left|\sum_{k=3}^b \binom{b}{k}(-a)^k \right|\\
       &\le \frac{a^2b^2}{2} +  \sum_{k=3}^b \binom{b}{k}(-a)^k \\
        &\le \frac{a^2b^2}{2} +  \sum_{k=3}^b (ab)^k \\
        &\le\frac{a^2b^2}{2} + \frac{a^3b^3}{1 - ab} \\
        &\le a^2b^2.
    \end{align*}
    Similarly,
    \begin{align*}
		\sum_{k=2}^b \binom{b}{k}(-a)^k &=  \frac{a^2b(b-1)}{2} + \sum_{k=3}^b \binom{b}{k}(-a)^k \\
		%
		&= \frac{a^2b^2}{2} - \frac{a^2b}{2}  + \sum_{k=3}^b \binom{b}{k}(-a)^k \\
		&\ge \frac{a^2b^2}{2} - \frac{a^2b}{2} -  \sum_{k=3}^b (ab)^k \\
		%
		&= \frac{a^2b^2}{2} - \frac{a^3b^3}{1 - ab} - \frac{a^2b}{2}\\
		%
		&\ge 0.
    \end{align*}
\end{proof}

\textbf{Proof of Theorem \ref{thm:neg}}.
Let $m\ge5$. Choose any $n > 1$ such that $\frac{\sqrt{n}}{\log(n)} \ge m \ge 2\log(n) + 2$. 
Define $\mathcal{D}$ as follows: for $u_{ij} \sim \mathcal{D}$,
\[
    u_{ij} = 
    \begin{dcases}
        n^4m & \text{ w.p. } \tfrac{1}{n^2m} \\
        n & \text{ w.p. } p := e^{-\log(m)/m} - \tfrac{1}{n^2m}\\
        1 & \text{ w.p. } q := 1 - e^{-\log(m)/m}.
    \end{dcases}
\]
Draw $m$ samples from $\mathcal{D}$ and denote them $X_{(1)},\ldots,X_{(m)}$, in increasing order.
The expectation of the largest sample is:
\begin{align*}
    \E[X_{(m)}] &= \Pr(X_{(m)} = 1) + \Pr(X_{(m)} = n)\cdot n + \Pr(X_{(m)} = n^4m)\cdot n^4m \\
    &= q^m + \left(\left(1-\tfrac{1}{n^2m}\right)^m - q^m\right)n + \left(1-\left(1-\tfrac{1}{n^2m}\right)^m\right)n^4m \\
    &\ge q^m + \left(\left(1-\tfrac{1}{n^2m}\right)^m - q^m\right)n + \left(1-\left(1-\tfrac{1}{n^2} +  \tfrac{1}{n^4}\right)\right)n^4m \\
    &= q^m + \left(\left(1-\tfrac{1}{n^2m}\right)^m - q^m\right)n + n^2m - m\\
    &\ge n^2m  -m,
\end{align*}
where we used \Cref{lem:atothebbounds} and the fact that $1-1/n^2 m \geq q$. 

For every $k < m$, we have that
\begin{align*}
    \E[X_{(k)}] &\le \E[X_{(m-1)}] \\
    &=  \Pr(X_{(m-1)} = 1) + \Pr(X_{(m-1)} = n)\cdot n + \Pr(X_{(m-1)} = n^4m)\cdot n^4m \\
    &\le n\Pr(X_{(m-1)} \ne n^4m) + \left(1-\left(1-\tfrac{1}{n^2m}\right)^{m}-m\left(1-\tfrac{1}{n^2m}\right)^{m-1}\left(\tfrac{1}{n^2m} \right)\right)n^4m \\
    &\le n + \left(\tfrac{1}{n^2}-\left(1-\tfrac{m-1}{n^2m}\right)\left(\tfrac{1}{n^2}\right)\right)n^4m \\
    &\le n + 2m,
\end{align*}
where again we used \Cref{lem:atothebbounds}.

Combining these two inequalities, we have that $\E[X_{(m)}] > n\E[X_{(k)}]$ for every $k$. Therefore, one voter ranking a chosen alternative first has higher expected utility than all $n$ voters ranking a chosen alternative second. This implies that if there is a unique alternative that is ranked first by the most voters, then that alternative is the unique expected welfare maximizing alternative.

We consider the following preference profile. Alternative $1$ is ranked first by $\frac{n}{m-1} + 1$ voters and ranked $m^{th}$ by $n - (\frac{n}{m-1} + 1) = n \cdot \frac{m-2}{m-1} - 1$ voters. Alternative $2$ is ranked second by all $n$ voters. Finally, all other alternatives are ranked first by at most $\frac{n}{m-1}$ voters.

In this construction, alternative $1$ has the most first place ranks and therefore is the unique expected welfare maximizing alternative. We now show that 
\[
    \E[\dist(1, \bsigma)] \le O\left(\frac{\E[\dist(2, \bsigma)]}{m}\right).
\]
Let $\mathcal{E}_1$ be the event that no voter has utility $n^4m$ for any alternative.  By \Cref{lem:atothebbounds}, we have that
\[
    \Pr(\mathcal{E}_1) = \left(1-\tfrac{1}{n^2m}\right)^{nm} \ge 1 - \tfrac{1}{n}.
\]
Let $\mathcal{E}_2$ be the event that every voter has utility at least $n$ for alternative $2$. Under event $\mathcal{E}_2$, the total welfare of alternative $2$ is at least $\SW(2, \bsigma) \geq n^2$. We have that
\begin{align*}
    \Pr(\mathcal{E}_2) &= \Pr(X_{(m-1)} \geq n)^n \\
    &\geq \Pr(X_{(m-1)} = n)^n \\
    &= \left(1 - q^m - mq^{m-1}(1-q) \right)^n \\
    & \ge \left( 1- q^m - mq^{m-1}\right)^n \\
    & \ge \left( 1- \left(\frac{\log(m)}{m}\right)^m - m\left(\frac{\log(m)}{m}\right)^{m-1}\right)^n \\
    & \ge \left( 1- \left(\frac{\log(m)}{m}\right)^m- \left(\frac{(m)^{1/(m-1)}\log(m)}{m}\right)^{m-1}\right)^n \\
    & \ge \left( 1- \left(\frac{1}{2}\right)^m- \left(\frac{1}{2}\right)^{m-1}\right)^n \\
    & \ge \left( 1- \frac{1}{n^2}\right)^n \\
    &\ge 1 - \frac{1}{n},
\end{align*}
where we simplified using that $q \le \frac{\log(m)}{m}$, $m \ge 5$, and $m \ge 2\log(n) + 2$.

We finally want to establish a tighter upper bound the typical utility of alternative 1 than event $\mathcal{E}_1$ alone provides. Let $N_1$ be the number of voters, among the $n \cdot \frac{m-2}{m-1} - 1$ voters that ranked alternative 1 in last place, who have utility strictly greater than $1$ for alternative $1$. Then let $\mathcal{E}_3$ be the event that:
\[
    N_1 \le \tfrac{1}{m} (n \cdot \tfrac{m-2}{m-1} - 1) + \log(n)\sqrt{n}.
\]
We will show $\mathcal{E}_3$ is also likely. 
To calculate $\Pr(\mathcal{E}_3)$, note that by definition of the probability $p$,
\[
    \Pr(X_{(1)} > 1) = \left(p+\tfrac{1}{n^2m}\right)^m = \left(m^{-1/m}\right)^m = \tfrac{1}{m}.
\]
Therefore, $N_1 \sim Bin(\frac{1}{m}, n \cdot \frac{m-2}{m-1} - 1)$. Applying Hoeffding's inequality to this random variable gives:
\begin{align*}
\Pr(\mathcal{E}_3)  &= 1 - \Pr\left(N_1 \ge \tfrac{1}{m} (n \cdot \tfrac{m-2}{m-1} - 1) + \log(n)\sqrt{n}\right) \\
&= 1 - \Pr\left(N_1 - \E[N_1] \ge \log(n)\sqrt{n}\right) \\
&\ge 1 - \exp\bigl(-2( \log(n)\sqrt{n})^2/( n \cdot \tfrac{m-2}{m-1} - 1)\bigr) \\
&\ge 1 - \exp(-2( \log(n)\sqrt{n})^2/n) \\
&= 1 - \exp(-2\log^2(n)) \\
&\ge  1-\tfrac{1}{n}.
\end{align*}

Define $\mathcal{E} := \mathcal{E}_1 \cap \mathcal{E}_2 \cap \mathcal{E}_3$. By inclusion/exclusion and a union bound, 
\begin{align*}
    \Pr(\mathcal{E}) &= 1 - \Pr(\neg \mathcal{E}_1 \cup \neg \mathcal{E}_2 \cup  \neg \mathcal{E}_3) \\
    &\ge 1- \Pr(\neg \mathcal{E}_1) - \Pr(\neg \mathcal{E}_2) - \Pr(\neg \mathcal{E}_3) \\
    &\ge 1-\frac{3}{n}.
\end{align*}
We consider the social welfare of alternatives $1$ and $2$ under event $\mathcal{E}$ to obtain bounds on their respective expected distributional distortions.

Event $\mathcal{E}_3$ implies that the total number of voters that have utility greater than $1$ for alternative $1$ (including the $\frac{n}{m-1} + 1$ voters who rank alternative $1$ first) is at most:
\[\tfrac{1}{m} \left(n \cdot \tfrac{m-2}{m-1} - 1\right) + \log(n)\sqrt{n} + \tfrac{n}{m-1} + 1.\] 

Under event $\mathcal{E}_1$, no voter has utility greater than $n$ for any alternative. Therefore, every voter has utility either $1$ or $n$ for alternative $1$. Since we have an upper bound on the number of voters that have utility $n$ for alternative $1$, and trivially at most $n$ voters have utility $1$ for alternative $1$, we upper bound the total social welfare for alternative $1$ by:
\begin{align*}
        \SW(1, \bsigma) &\le n\cdot \left(\tfrac{1}{m} \left(n \cdot \tfrac{m-2}{m-1} - 1\right) + \log(n)\sqrt{n} + \tfrac{n}{m-1} + 1\right) + 1 \cdot n 
        \\
        &\le \tfrac{n^2}{m} + \log(n)n^{3/2} + \tfrac{2n^2}{m} + n\\
        &\le \tfrac{4n^2}{m} + \log(n)n^{3/2}.
\end{align*}

Combining this with the fact that $\SW(2, \bsigma) \geq n^2$ under event $\mathcal{E}_2$, we get that the distributional distortion under event $\mathcal{E}$ is at most the following, using that $m \le \frac{\sqrt{n}}{\log(n)}$:
\[   
    \frac{\frac{4n^2}{m} + \log(n)n^{3/2} }{n^2} = \frac{4}{m} + \frac{\log(n)}{\sqrt{n}} \le \frac{5}{m}. 
\] 
Since $\Pr(\mathcal{E}) \ge 1-\frac{3}{n}$,  the distributional distortion of alternative $1$ is upper bounded as follows:
\[
    \E[\dist(1, \bsigma)] \le \left(1-\tfrac{3}{n}\right)\cdot \tfrac{5}{m} + \tfrac{3}{n} \cdot 1\le \tfrac{8}{m}. 
\]
Under event $\mathcal{E}$, alternative $2$ has total social welfare of $n^2$ and the max social welfare of any alternative is $n^2$. This implies that alternative $2$ has distributional distortion $1$. The expected distributional distortion of alternative $2$ is thus lower bounded as follows:
\[
    \E[\dist(2, \bsigma)] \ge \left(1-\frac{3}{n}\right)\cdot 1 + \frac{3}{n} \cdot 0 \ge \frac{1}{2}.
\]
Therefore, 
\begin{align*}
    \E[\dist(\ewmr, \bsigma)] &= \E[\dist(1, \bsigma)] \\
    &\le \tfrac{16}{m}\E[\dist(2, \bsigma)] \\
    &\le \tfrac{16}{m}\E[\dist(\edmr, \bsigma)]. 
\end{align*}

Note that while this distribution is not supported on $[0,1]$, simply scaling the values of the distribution by $\frac{1}{n^4m}$ will make the distribution supported on $[0,1]$. Furthermore, expected distortion is invariant to scaling the distribution, and therefore the result still holds.
$\qedsymbol$

\section{Proof of Theorem~\ref{thm:pos}}\label{app:proof_of_pos}

\begin{lemma} \label{lem:bdd_dist_IDSW_bound}
    Suppose the distribution $\mathcal{D}$ has mean $\mu$ and is supported on $(0, 1]$. Then the expected distributional distortion of the alternative selected by the expected welfare maximizing rule is at least $\mu$. Furthermore, the expected welfare of the expected welfare maximizing alternative is at least $n\mu$.
\end{lemma}

\begin{proof}
    First, note that by the linearity of expectation $\E[\SW(j, \bsigma)] = \sum_{i=1}^n \E[u_{ij}]= n\mu$ for all $j$. 
    Therefore, the alternative selected by the expected welfare maximizing rule must have expected social welfare of at least $n\mu$.
    Therefore, using the fact that no alternative can have social welfare of greater than $nB$,
    \begin{align*}
        \E[\dist(\ewmr, \bsigma)] &= \E\left[\frac{\SW(\ewmr, \bsigma)}{\max_j \SW(j, \bsigma)}\right] \\
        &\ge \E\left[\frac{\SW(\ewmr, \bsigma)}{n}\right] \\
        &= \frac{\E[\SW(\ewmr, \bsigma)]}{n} \\
        &\ge \frac{n\mu}{n} \\
        &= \mu.
    \end{align*}
\end{proof}

The below is a purely technical lemma.
\begin{lemma} \label{lem:order_stat_variance_bound}
	If $X_1,...,X_m$ are i.i.d. draws from a differentiable distribution with cdf $F$. 
	Suppose that $F$ satisfies the condition that there is some $c$ such that $\inf_{x} \frac{dF(x)}{dx} = c > 0$.
	Then for all $s_\epsilon > 0$, there exists $M_1$ such that for any $m > M_1$ and for any $j$,
	\[Var(X_{(j)}) \le s_\epsilon^2.\]
\end{lemma}

\begin{proof}
    Let $F$ be the cdf of $\mathcal{D}$ and let $F_m$ be the empirical cdf from $m$ samples. Let $|F - F_m| = \sup_x |F(x) - F_m(x)|$. The iterated logarithm law of Smirnov (see \cite{Smirnov44, Chung49} ) states that:
    \[
        \Pr\left(\limsup_{m \longrightarrow \infty} \frac{\sqrt{m}|F_m - F|}{(2\log\log(m))^{1/2}} = c \le \frac{1}{2}\right) = 1.
    \]
    A consequence of this is that for any $\delta > 0$, there exists an $M_1$ such that for all $m \ge M_1$:
    \[
        \Pr\left(|F_m - F| \le \frac{(2\log\log(m))^{1/2}}{\sqrt{m}}\right) \ge 1 - \delta
    \]
    Note that because $F$ is differentiable and $\inf_{x \in [0,1]} F'(x) \ge c > 0$, this implies that
    \[
        \Pr\left(|F_m^{-1} - F^{-1}| \le \frac{(2\log\log(m))^{1/2}}{c\sqrt{m}}\right) \ge 1 - \delta,
    \]
    where $F^{-1}$ denotes the inverse of the cdf.
    Finally, we note that the $j^{th}$ order statistic is equivalent to $F_m^{-1}(\frac{j}{m})$, and so we have that
    \[
        \Pr\left(|X_{(j)} - F^{-1}(j/m)| \le \frac{(2\log\log(m))^{1/2}}{c\sqrt{m}}\right) \ge 1 - \delta.
    \]
    Using the fact that $X_{(j)}$ is supported on $(0,1]$, this gives that the variance of $X_{(j)}$ can be bounded as
    \[\Var(X_{(j)}) \le \left(\frac{(2\log\log(m))^{1/2}}{c\sqrt{m}}\right)^2 + \delta \le s_\epsilon^2,\]
    where we take $\delta = \frac{s_\epsilon^2}{2}$ and sufficiently large $m$.
\end{proof}

\textbf{Proof of Theorem \ref{thm:pos}}.
    Recall that $\ewmr(\bsigma)$ is the expected welfare maximizing alternative. Let $n \ge n_0$, where $n_0$ is the solution to the equation $\frac{\log(n)}{\sqrt{\mu n}} = \epsilon_0$. By \Cref{lem:bdd_dist_IDSW_bound}, the expected welfare maximizing alternative satisfies $\E[\SW(\ewmr, \bsigma)] \ge n\mu$. Furthermore, note that the social welfare of any alternative $j$ can be represented as $\SW(j, \bsigma) = \sum_{i=1}^n u_{ij}$ where $u_{ij}$ are $n$ i.i.d. random variables that are supported on $(0,1]$. Therefore, we can apply Hoeffding's theorem to get the following:
    \begin{align*}
        &\Pr(\SW(\ewmr, \bsigma) \le (1-\epsilon)\E[\SW(\ewmr, \bsigma)]) \\
        &= \Pr(\SW(\ewmr, \bsigma) - \E[\SW(\ewmr, \bsigma)] \le - \epsilon \E[\SW(\ewmr, \bsigma)]) \\
        & \le \Pr(\SW(\ewmr, \bsigma) - \E[\SW(\ewmr, \bsigma)] \le - \epsilon n\mu)\\
        &\le e^{-2(\epsilon n\mu)^2/n}\\
        &\le e^{-2\epsilon^2n\mu^2}.
    \end{align*}
    For any $j \ne \ewmr(\bsigma)$, we must have $\E[\SW(j, \bsigma)] \le \E[\SW(\ewmr, \bsigma)]$. Therefore:
    \begin{align*}
        &\Pr(\SW(j, \bsigma) \ge (1+\epsilon)\E[\SW(\ewmr, \bsigma)]) \\
        &\le \Pr(\SW(j, \bsigma) \geq \E[\SW(j, \bsigma)] + \epsilon \E[\SW(\ewmr, \bsigma)])\\
        &= \Pr(\SW(j, \bsigma) - \E[\SW(j, \bsigma)] \ge \epsilon \E[\SW(\ewmr, \bsigma)]) \\
        & \le \Pr(\SW(j, \bsigma) - \E[\SW(j, \bsigma)] \ge \epsilon n\mu)\\
        &\le e^{-2(\epsilon n\mu)^2/n}\\
        &\le e^{-2\epsilon^2n\mu^2}.
    \end{align*}
    Let $\mathcal{E}$ be the event that the welfare of the $\ewmr(\sigma)$ alternative is not too small, and that no other alternative has unusually large welfare; $\SW(\ewmr, \bsigma) \ge (1-\epsilon)\E[\SW(\ewmr, \bsigma)]$ and that for all $j \ne \ewmr(\bsigma)$, $\SW(j, \bsigma) \leq (1+\epsilon)\E[\SW(\ewmr, \bsigma)]$. Mathematically, 
    \[
        \mathcal{E} = \big\{\SW(\ewmr, \bsigma) \geq (1-\epsilon)\E[\SW(\ewmr, \bsigma)]\big\} \cap \big\{\forall j :  \SW(j, \bsigma) \leq (1+\epsilon)\E[\SW(\ewmr, \bsigma)]\big\}.
    \]
    Using the two results above, the probability of the event $\mathcal{E}$ can be lower bounded by the following:
    \[
        \Pr(\mathcal{E}) \ge 1 - e^{-2\epsilon^2n\mu^2} - e^{-2\epsilon^2n\mu^2} = 1 - 2e^{-2\epsilon^2n\mu^2}  
    \]
    Fix any $j$. Under event $\mathcal{E}$, the distributional distortion of this alternative satisfies the following inequality:
    \begin{align*}
        \dist(j, \bsigma) &= \frac{\SW(j, \bsigma)}{\max_j \SW(j, \bsigma)} \\
        &\le  \frac{(1 + \epsilon)\E[\SW(\ewmr, \bsigma)]}{\max_j \SW(j, \bsigma)} \\
        &\leq \frac{1+\epsilon}{1-\epsilon} \cdot \frac{\SW(\ewmr, \bsigma)}{\max_j \SW(j, \bsigma)} \\
        &= \frac{1 + \epsilon}{1 - \epsilon} \cdot \dist(\ewmr, \bsigma)
    \end{align*}    
    Under event $\neg \mathcal{E}$, the distributional distortion of $j$ is at most $1$ by definition. Therefore, we can upper bound the expected distributional distortion of $j$ relative to the expected distributional distortion of $\ewmr(\bsigma)$ as follows:
    \begin{align*}
        \E[\dist(j, \bsigma)] &= \Pr(\mathcal{E}) \cdot \E[\dist(j, \bsigma) | \: \mathcal{E}] + \Pr(\neg \mathcal{E}) \cdot \E[\dist(j, \bsigma) | \: \neg \mathcal{E}] \\
        %
        &\leq \tfrac{1+\epsilon}{1-\epsilon} \cdot \Pr(\mathcal{E}) \cdot \E[\dist(\ewmr, \bsigma) | \: \mathcal{E}] + 2e^{-2\epsilon^2n\mu^2} \\
        %
        &\leq \tfrac{1+\epsilon}{1-\epsilon} \cdot \Big(\Pr(\mathcal{E}) \cdot  \E[\dist(\ewmr, \bsigma) | \: \mathcal{E}] + \Pr(\neg\mathcal{E}) \cdot  \E[\dist(\ewmr, \bsigma) | \: \neg\mathcal{E}]\Big) + 2e^{-2\epsilon^2n\mu^2} \\
        %
        &\leq \tfrac{1+\epsilon}{1-\epsilon} \cdot \E[\dist(\ewmr, \bsigma)] + 2e^{-2\epsilon^2n\mu^2} \cdot \tfrac{1}{\mu} \E[\dist(\ewmr, \bsigma)] \\
        %
        &\leq \left(\tfrac{1+\epsilon}{1-\epsilon} + \tfrac{2}{\mu} \cdot e^{-2\epsilon^2n\mu} \right)\E[\dist(\ewmr, \bsigma)].
    \end{align*}
    Take $\epsilon = \frac{\epsilon_0}{8} \leq \frac{1}{2}$, which is equal to $ \frac{\log(n)}{2\sqrt{\mu n}}$ by our choice of $n$. Then:
    \begin{align*}
        \tfrac{1+\epsilon}{1-\epsilon} + \tfrac{2}{\mu}e^{-2\epsilon^2n\mu}  &\le 1 + 4\epsilon + \tfrac{2}{\mu}e^{-2\epsilon^2n\mu} \\
        &\le 1 + \tfrac{\epsilon_0}{2} + \tfrac{2}{\mu}\sqrt{n}^{-\log(n)} \\
        &\le 1 + \epsilon_0.
    \end{align*}
    We have shown that for all $j$
    \[
        \E[\dist(j, \bsigma)] \le (1+\epsilon_0)\E[\dist(\ewmr, \bsigma)],
    \]
    and therefore,
    \[
        \E[\dist(\edmr, \bsigma)] = \max_j \E[\dist(j, \bsigma)] \le (1+\epsilon_0)\E[\dist(\ewmr, \bsigma)].
    \]
    \medskip
    We have shown that the expected social welfare maximizing rule is an $\epsilon$-approximation for the expected distributional distortion maximizing rule for sufficiently large $n$. We now show that the same holds for sufficiently large $m$ when $\mathcal{D}$ is continuous. The proof is very similar to the above, except that we use Chebyshev's inequality instead of Hoeffding's inequality. 
    
    Note that $\SW(j, \bsigma)$ is the sum of $n$ independent random variables, and let $s_\epsilon^2$ be an upper bound on the variance of any one of these random variables. We can use \Cref{lem:order_stat_variance_bound} to find a $m_0$ that is suitably large. Specifically, we choose $m_0$ such that $m \ge m_0$ implies $s_\epsilon^2 \le \frac{\epsilon_0^3\mu^3n}{256}$. 
    
    Because the variance of a sum of independent random variables is the sum of the variances, we can bound $\Var(\SW(j, \bsigma)) \le ns_\epsilon^2$. Applying Chebyshev's inequality then yields:
    \begin{align*}
        &\Pr(\SW(\ewmr, \bsigma) \le (1-\epsilon)\E[\SW(\ewmr, \bsigma)]) \\&= \Pr(\SW(\ewmr, \bsigma) - \E[\SW(\ewmr, \bsigma)] \le - \epsilon \E[\SW(\ewmr, \bsigma)]) \\
        & \le \Pr(\SW(\ewmr, \bsigma) - \E[\SW(\ewmr, \bsigma)] \le - \epsilon n\mu)\\
        &\le \frac{ns_\epsilon^2}{(\epsilon n \mu)^2}\\
        &= \frac{s_\epsilon^2}{\epsilon^2\mu^2n}.
    \end{align*}
    For any $j \ne \ewmr(\bsigma)$, we must have $\E[\SW(j, \bsigma)] \le \E[\SW(\ewmr, \bsigma)]$, and therefore:
    \begin{align*}
        &\Pr(\SW(j, \bsigma) \ge (1+\epsilon)\E[\SW(\ewmr, \bsigma)])\\
        &\le \Pr(\SW(j, \bsigma) \geq \E[\SW(j, \bsigma)] + \epsilon \E[\SW(\ewmr, \bsigma)])\\
        &= \Pr(\SW(j, \bsigma) - E[\SW(j, \bsigma)] \ge \epsilon \E[\SW(\ewmr, \bsigma)]) \\
        & \le \Pr(\SW(j, \bsigma) - \E[\SW(j, \bsigma)] \ge \epsilon n\mu)\\
        &\le \frac{ns_\epsilon^2}{(\epsilon n \mu)^2}\\
        &= \frac{s_\epsilon^2}{\epsilon^2\mu^2n}.
    \end{align*}
    Using the same logic as in the first part of the proof, this means that we have
    \begin{align*}
        \E[\dist(j, \bsigma)] &\le \left(\frac{1+\epsilon}{1-\epsilon} +\frac{2s_\epsilon^2}{\epsilon^2\mu^3n}\right)\E[\dist(\ewmr, \bsigma)]
    \end{align*}
    We can upper bound this by taking $\epsilon = \frac{\epsilon_0}{8}$ to get:
    \begin{align*}
        \frac{1+\epsilon}{1-\epsilon} + \frac{2s_\epsilon^2}{\epsilon^2\mu^3n}  &\le 1 + 4\epsilon +  \frac{2s_\epsilon^2}{\epsilon^2\mu^3n}  \\
        &\le 1 + \frac{\epsilon_0}{2} +  \frac{128s_\epsilon^2}{\epsilon_0^2\mu^3n}  \\        
        &\le 1 + \epsilon_0.
    \end{align*}
    As in the first section of the proof, this implies that:
    \[
        \E[\dist(\edmr, \bsigma)] = \max_j \E[\dist(j, \bsigma)] \le (1+\epsilon_0)\E[\dist(\ewmr, \bsigma)].
    \]
$\qedsymbol$
